Controllable Generation from Pre-trained Language Models via Inverse Prompting

Large-scale pre-trained language models have demonstrated strong capabilities of generating realistic text. However, it remains challenging to control the generation results. Previous approaches such as prompting are far from sufficient, which limits the usage of language models. To tackle this challenge, we propose an innovative method, inverse prompting, to better control text generation. The core idea of inverse prompting is to use generated text to inversely predict the prompt during beam search, which enhances the relevance between the prompt and the generated text and provides better controllability. Empirically, we pre-train a large-scale Chinese language model to perform a systematic study using human evaluation on the tasks of open-domain poem generation and open-domain long-form question answering. Our results show that our proposed method substantially outperforms the baselines and that our generation quality is close to human performance on some of the tasks. Narrators can try our poem generation demo at https://pretrain.aminer.cn/apps/poetry.html, while our QA demo can be found at https://pretrain.aminer.cn/app/qa. For researchers, the code is provided in https://github.com/THUDM/InversePrompting.

==> 5.a.turing.tex <==
\subsection{Turing Test Evaluation}

\subsubsection{Background}

Currently, the evaluation for large pre-training models mainly relies on downstream tasks. For example, BERT~\cite{devlin2018bert} uses a variety of natural language processing tasks to evident its superior capability on understanding human language, such as Question Answering or Natural Language Inference. Other LM-based generation models like GPT-3~\cite{brown2020language} make evaluations on some more generation tasks, such as completing the last words of long paragraphs, selecting correct endings for stories or translation.

Running evaluations on existing materials like expert annotated corpus or automatically constructed datasets makes it convenient for researchers to reproduce the results and compare performances between different methods. However, it requires human knowledge and extra efforts to find suitable materials and build reasonable benchmark tests, which is extremely hard for many online applications targeting at some specific domains. Thus, we designed new evaluation method for the online applications in our proposed framework.


\subsubsection{Imitating Human Being}

In our framework, several pretrain-based online applications share the same target to generate human-like contents. In \textit{Personalized Question Answer}, the model is expected to answer open questions with the specified personality or character. In \textit{AI-Poet}, we want the model to generate poems in old fashions like human poets thousands years ago. \textit{Creating images from texts} is another application that related to the general purpose of imitating human. For example, given the title and description of one oil painting, the more the generated painting is similar to man-made, the better capability the model is presumably to have. Thus, we borrowed the idea of Turing test to make evaluations for generation-based applications.

Turing test, originally called the imitation game, was first introducted by Alan Turing in 1950~\cite{turing2009computing}. It is used to test a machine's ability to exhibit intelligent behaviours like human beings. While there are different intepretations for the intention of Turing test, it is commonly understood that if a machine can generate human-like responses, which makes it indistinguishable from real human beings for evaluators, then we can say this machine shows some ability of imitating human.

As for our framework, different from the Turing test defined by Alan Turing, which requires the machine to imitate human beings during conversation with evaluators, we designed a pseudo-Turing test for our applications that generate human-like contents.

\begin{figure}[h]
  \includegraphics[width=0.48\textwidth, trim={0 0 0 1cm}, clip]{ai-poet.png}
  \caption{The structure of our proposed imitation game on \textit{AI-Poet}. First, we take one real poem created by human poet thousand years ago. Then, we feed the title of one poem to the AI agent and let it generate one poem. Finally, we ask the user to distinguish the original human-made poem from the generated poem.}
\label{fig:ai-poet}
\end{figure}

\subsubsection{Methodology}

In our imitation game, for each model that generates human-like contents, we treated it as one \textit{AI-agent}, denoted as $\mathcal{A}$. To test the performance of one \textit{AI-agent}, we invited evaluators to distinguish $n$ groups of generated contents. Each group is given a pair of content $<h_c,a_c>$, where $h_c$ is the content generated by human under context $c$ and $a_c$ is the one generated by \textit{AI-agent} $\mathcal{A}$.

To explain the designed game straightforwardly, we will take the \textit{AI-Poet} application as an example in the following parts.  For \textit{AI-Poet}\footnote{\url{https://turing-poet.aminer.cn/index.html}}, we took the title, author name, the number of sentences and the number of words in each sentence from one human-made poem as context $c$, asked the agent $\mathcal{A}$ to generate a new poem $a_c$ for it. The sentences in original poem is treated as $h_c$. Evaluators are requested to choose which one is made by human poet as shown in Figure~\ref{fig:ai-poet}.

After games, we collected all the answers and calculated the proportion of selected poems made by \textit{AI-agent}. The results were used for evaluating pre-training model performance on the target application. If the proportion of selected poems made by \textit{AI-agent} reaches over 50\%, the model can be seen as passing our pseudo-Turing test.

\subsubsection{Game Details}

As our online evaluation relies on the feedback from real human evaluators, we designed several more interesting modes for the game beyond the basic pseudo-Turing test described above, to attract more users participate in our tests. We named these modes according to their difficulties. The standard test is named as ``easy''. A simple example of this mode is illustrated in Figure~\ref{fig:turing-poet}.

\begin{figure}[h]
  \includegraphics[width=0.48\textwidth, trim={0 0 0 1cm}, clip]{poetry.png}
  \caption{An example of the imitation game for \textit{AI-Poet}. The left side is the game UI and the right side is the translation. Users are requested to selected one poem which is likely to be made by human.}
\label{fig:turing-poet}
\end{figure}

Currently, our online \textit{AI-agent} is not always intelligent enough to cheat human evaluators. We added another two challenging modes named ``hard'' and ``lunatic''. The former one asks users to distinguish the human-made poem from two other AI-made poems with limited time. The latter one sometimes provides three AI-mode poems and users need to make empty choice in this situation. The time limit is reduced by one third as well.

Another ``extra'' mode is added to make comparisons between different \textit{AI-agent}s. Three choices are given to users with one human-made poem and two poems generated by different \textit{AI-agent}s. Through the final click through rates, we can not only see how close \textit{AI-agent}s are close to human but also make comparisons between various \textit{AI-agent}s.

Besides, test cases are pre-generated and form a test case bank. Each time an user starts a game, we randomly select $n$ test cases for the user.

While the added three modes are more challenging for users, it is noticeable that the results from these modes can reach different conclusions, which needs to be carefully intepretated. For example, in ``hard'' mode, two incorrect poems made by the same \textit{AI-agent} might sometimes share some similarities (such as two generated poems have the same first sentence) that are easily observed, which provides extra information for user to judge. As a result, we mainly evaluate on results from ``easy'' mode (the basic test) and ``extra'' mode and use the other two modes as supplementary.

\subsubsection{Evaluation Results}

For \textit{AI-Poet}, we opened the imitation game for about one month and over 1,300 users participated in the game. For the last two weeks, we tested two different \textit{AI-agent} on our game platform. One agent is built with our \textit{Pretrained} model as described above and the other is built based on \textit{Jiuge}~\cite{yi2020mixpoet}, one of the state-of-the-art Chinese poetry generation model\footnote{\url{http://jiuge.thunlp.org/}}.

For ``easy'' mode, each test case contains one poem generated by \textit{AI-agent} and the other poem created by human poet. To test the performance difference between two different \textit{AI-agent}s, for each test case, we randomly select one agent to generate a poem. For ``extra'' mode, we followed the introduction above and created testcases with one poem generated by human, one by pretrained model and one by Jiuge.

We cleaned up the game records by removing records that user did not make any choice. Finally, we collected 1,261 ``easy'' mode records and 1,095 ``extra'' mode records. The details are listed in Table~\ref{tab:turing-test-records}.

\begin{table}[ht]
  \centering
  \vcaption{The details of collected imitation game records, including the number of records in the test, the number of selected times, click through rate (CTR) and the average response time. \textit{Pretrain} means the \textit{AI-agent} developed based on our pretrain model. \textit{Jiuge} and \textit{Human} represent poems generated by \textit{Jiuge}'s model and human poets respectively.}
  \label{tab:turing-test-records}
  \begin{tabular}{ccccc}
    \toprule
    & Records & Selected & CTR & Avg. Time (sec) \\
    \midrule
    \multicolumn{5}{l}{\textit{``easy'' mode Pretrain-Human test}} \\
    \quad Pretrain & 610 & 280 & 45.9\% & 23.29 \\
    \quad Human & 610 & 330 & 54.1\% & 32.09 \\
    \cdashline{1-5}
    % \midrule
    \multicolumn{5}{l}{\textit{``easy'' mode Jiuge-Human test}} \\
    \quad Jiuge & 621 & 310 & 49.9\% & 26.97 \\
    \quad Human & 621 & 311 & 50.1\% & 27.22 \\
    \cdashline{1-5}
    % \midrule
    \multicolumn{5}{l}{\textit{``extra'' mode test}} \\
    \quad Pretrain & 1,095 & 321 & 29.3\% & 17.89 \\
    \quad Jiuge & 1,095 & 382 & 34.9\% & 19.46 \\
    \quad Human & 1,095 & 392 & 35.8\% & 19.92 \\
    \bottomrule
  \end{tabular}
\end{table}

From the click through rates we could see that there is some distance for our pretrained model based \textit{AI-agent} to reach the level of human poets. But it is also not very easy and obvious to pick out the human-made poem without careful consideration. On the other hand, the Jiuge system, which is dedicated on generating poems, turns out to be fairly indistinguishable. The average time cost seems to indicate that a longer-time consideration might be helpful to distinguish AI-made poets from human-made ones.

\subsubsection{Discussion}

In the work of \textit{Jiuge}~\cite{yi2020mixpoet}, the authors invited human annotators to evaluate the generated poems through several different human-defined quality metrics, such as fluency, context coherence or topic relevance. Compared to their evaluation methods, our imitation game requires much less expert knowledge and has a different goal. The evaluation goal in \textit{Jiuge} is to judge which model generate higher quality poems while our evaluation goal is to tell whether tested model can act like human poets. Thus, instead of replacing previous evaluation methods, our method provides another view of model performance in a cheaper and more straightforward way.

Despite the drawback that the reproduction of online evaluation can yield various results due to the variance of testers, the proposed imitation game is particularly easy to be applied on other generation-based applications, such as personalized question answering or text-based image creation. In addition, as our pretrain-based online applications always face users directly, the online evaluation can be integrated in our standardized framework without too much efforts.

==> abstract_for_submission.tex <==
Large-scale pretrained language models have demonstrated strong capabilities of generating realistic text. However, it remains challenging to control the generation results. Previous approaches such as prompting are far from sufficient, which limits the usage of language models. To tackle this challenge, we propose an innovative method, inverse prompting, to better control text generation. The core idea of inverse prompting is to use generated text to inversely predict the prompt during beam search, which enhances the relevance between the prompt and the generated text and provides better controllabilty. Empirically, we pretrain a large-scale Chinese language model to perform a systematic study using human evaluation on the tasks of open-domain poem generation and open-domain long-form question answering. Our results show that our proposed method substantially outperforms the baselines and that our generation quality is comparable to human on some of the tasks.

==> evaluation.tex <==
\clearpage

\section{Evaluation}

\subsection{Background}

Currently, the evaluation for large pre-training models mainly relies on downstream tasks. For example, BERT~\cite{devlin2018bert} uses a variety of natural language processing tasks to evident its superior capability on understanding human language, such as Question Answering or Natural Language Inference. Other LM-based generation models like GPT-3~\cite{brown2020language} make evaluations on some more generation tasks, such as completing the last words of long paragraphs, selecting correct endings for stories or translation.

Running evaluations on existing materials like expert annotated corpus or automatically constructed datasets makes it convenient for researchers to reproduce the results and compare performances between different methods. However, it requires human knowledge and extra efforts to find suitable materials and build reasonable benchmark tests, which is extremely hard for many online applications targeting at some specific domains. Thus, we designed new evaluation method for the online applications in our proposed framework.


\subsection{Imitating Human Being}

In our framework, several pretrain-based online applications share the same target to generate human-like contents. In \textit{Personalized Question Answer}, the model is expected to answer open questions with the specified personality or character. In \textit{AI-Poet}, we want the model to generate poems in old fashions like human poets thousands years ago. \textit{Creating images from texts} is another application that related to the general purpose of imitating human. For example, given the title and description of one oil painting, the more the generated painting is similar to man-made, the better capability the model is presumably to have. Thus, we borrowed the idea of Turing test to make evaluations for generation-based applications.

Turing test, originally called the imitation game, was first introducted by Alan Turing in 1950~\cite{turing2009computing}. It is used to test a machine's ability to exhibit intelligent behaviours like human beings. While there are different intepretations for the intention of Turing test, it is commonly understood that if a machine can generate human-like responses, which makes it indistinguishable from real human beings for evaluators, then we can say this machine shows some ability of imitating human.

As for our framework, different from the Turing test defined by Alan Turing, which requires the machine to imitate human beings during conversation with evaluators, we designed a pseudo-Turing test for our applications that generate human-like contents.

\begin{figure}[h]
  \includegraphics[width=0.48\textwidth, trim={0 0 0 1cm}, clip]{ai-poet.png}
  \caption{The structure of our proposed imitation game on \textit{AI-Poet}. First, we take one real poem created by human poet thousand years ago. Then, we feed the title of one poem to the AI agent and let it generate one poem. Finally, we ask the user to distinguish the original human-made poem from the generated poem.}
\label{fig:ai-poet}
\end{figure}

\subsection{Methodology}

In our imitation game, for each model that generates human-like contents, we treated it as one \textit{AI-agent}, denoted as $\mathcal{A}$. To test the performance of one \textit{AI-agent}, we invited evaluators to distinguish $n$ groups of generated contents. Each group is given a pair of content $<h_c,a_c>$, where $h_c$ is the content generated by human under context $c$ and $a_c$ is the one generated by \textit{AI-agent} $\mathcal{A}$.

To explain the designed game straightforwardly, we will take the \textit{AI-Poet} application as an example in the following parts.  For \textit{AI-Poet}\footnote{\url{https://turing-poet.aminer.cn/index.html}}, we took the title, author name, the number of sentences and the number of words in each sentence from one human-made poem as context $c$, asked the agent $\mathcal{A}$ to generate a new poem $a_c$ for it. The sentences in original poem is treated as $h_c$. Evaluators are requested to choose which one is made by human poet as shown in Figure~\ref{fig:ai-poet}.

After games, we collected all the answers and calculated the proportion of selected poems made by \textit{AI-agent}. The results were used for evaluating pre-training model performance on the target application. If the proportion of selected poems made by \textit{AI-agent} reaches over 50\%, the model can be seen as passing our pseudo-Turing test.

\subsection{Game Details}

As our online evaluation relies on the feedback from real human evaluators, we designed several more interesting modes for the game beyond the basic pseudo-Turing test described above, to attract more users participate in our tests. We named these modes according to their difficulties. The standard test is named as ``easy''. A simple example of this mode is illustrated in Figure~\ref{fig:turing-poet}.

\begin{figure}[h]
  \includegraphics[width=0.48\textwidth, trim={0 0 0 1cm}, clip]{poetry.png}
  \caption{An example of the imitation game for \textit{AI-Poet}. The left side is the game UI and the right side is the translation. Users are requested to selected one poem which is likely to be made by human.}
\label{fig:turing-poet}
\end{figure}

Currently, our online \textit{AI-agent} is not always intelligent enough to cheat human evaluators. We added another two challenging modes named ``hard'' and ``lunatic''. The former one asks users to distinguish the human-made poem from two other AI-made poems with limited time. The latter one sometimes provides three AI-mode poems and users need to make empty choice in this situation. The time limit is reduced by one third as well.

Another ``extra'' mode is added to make comparisons between different \textit{AI-agent}s. Three choices are given to users with one human-made poem and two poems generated by different \textit{AI-agent}s. Through the final click through rates, we can not only see how close \textit{AI-agent}s are close to human but also make comparisons between various \textit{AI-agent}s.

Besides, test cases are pre-generated and form a test case bank. Each time an user starts a game, we randomly select $n$ test cases for the user.

While the added three modes are more challenging for users, it is noticeable that the results from these modes can reach different conclusions, which needs to be carefully intepretated. For example, in ``hard'' mode, two incorrect poems made by the same \textit{AI-agent} might sometimes share some similarities (such as two generated poems have the same first sentence) that are easily observed, which provides extra information for user to judge. As a result, we mainly evaluate on results from ``easy'' mode (the basic test) and ``extra'' mode and use the other two modes as supplementary.

\subsection{Evaluation Results}

For \textit{AI-Poet}, we opened the imitation game for about one month and over 1,300 users participated in the game. For the last two weeks, we tested two different \textit{AI-agent} on our game platform. One agent is built with our \textit{Pretrained} model as described above and the other is built based on \textit{Jiuge}~\cite{yi2020mixpoet}, one of the state-of-the-art Chinese poetry generation model\footnote{\url{http://jiuge.thunlp.org/}}.

For ``easy'' mode, each test case contains one poem generated by \textit{AI-agent} and the other poem created by human poet. To test the performance difference between two different \textit{AI-agent}s, for each test case, we randomly select one agent to generate a poem. For ``extra'' mode, we followed the introduction above and created testcases with one poem generated by human, one by pretrained model and one by Jiuge.

We cleaned up the game records by removing records that user did not make any choice. Finally, we collected 1,261 ``easy'' mode records and 1,095 ``extra'' mode records. The details are listed in Table~\ref{tab:turing-test-records}.

\begin{table}[ht]
  \centering
  \vcaption{The details of collected imitation game records, including the number of records in the test, the number of selected times, click through rate (CTR) and the average response time. \textit{Pretrain} means the \textit{AI-agent} developed based on our pretrain model. \textit{Jiuge} and \textit{Human} represent poems generated by \textit{Jiuge}'s model and human poets respectively.}
  \label{tab:turing-test-records}
  \begin{tabular}{ccccc}
    \toprule
    & Records & Selected & CTR & Avg. Time (sec) \\
    \midrule
    \multicolumn{5}{l}{\textit{``easy'' mode Pretrain-Human test}} \\
    \quad Pretrain & 610 & 280 & 45.9\% & 23.29 \\
    \quad Human & 610 & 330 & 54.1\% & 32.09 \\
    \cdashline{1-5}
    % \midrule
    \multicolumn{5}{l}{\textit{``easy'' mode Jiuge-Human test}} \\
    \quad Jiuge & 621 & 310 & 49.9\% & 26.97 \\
    \quad Human & 621 & 311 & 50.1\% & 27.22 \\
    \cdashline{1-5}
    % \midrule
    \multicolumn{5}{l}{\textit{``extra'' mode test}} \\
    \quad Pretrain & 1,095 & 321 & 29.3\% & 17.89 \\
    \quad Jiuge & 1,095 & 382 & 34.9\% & 19.46 \\
    \quad Human & 1,095 & 392 & 35.8\% & 19.92 \\
    \bottomrule
  \end{tabular}
\end{table}

From the click through rates we could see that there is some distance for our pretrained model based \textit{AI-agent} to reach the level of human poets. But it is also not very easy and obvious to pick out the human-made poem without careful consideration. On the other hand, the Jiuge system, which is dedicated on generating poems, turns out to be fairly indistinguishable. The average time cost seems to indicate that a longer-time consideration might be helpful to distinguish AI-made poets from human-made ones.

\subsection{Discussion}

In the work of \textit{Jiuge}~\cite{yi2020mixpoet}, the authors invited human annotators to evaluate the generated poems through several different human-defined quality metrics, such as fluency, context coherence or topic relevance. Compared to their evaluation methods, our imitation game requires much less expert knowledge and has a different goal. The evaluation goal in \textit{Jiuge} is to judge which model generate higher quality poems while our evaluation goal is to tell whether tested model can act like human poets. Thus, instead of replacing previous evaluation methods, our method provides another view of model performance in a cheaper and more straightforward way.

Despite the drawback that the reproduction of online evaluation can yield various results due to the variance of testers, the proposed imitation game is particularly easy to be applied on other generation-based applications, such as personalized question answering or text-based image creation. In addition, as our pretrain-based online applications always face users directly, the online evaluation can be integrated in our standardized framework without too much efforts.

==> removed_tables.tex <==
\hide{
\begin{table}[ht]
    \tiny
    \centering
    \caption{An example showing how language models may fail to generate relevant contexts, and how \model prevents this mode decay from happening. }
    \vspace{-0.12in}
    \label{tab:example}
    \begin{tabular}{p{0.06\textwidth}p{0.37\textwidth}}
    
    \toprule
    Question & 有什么优美的词可以形容愤怒?
    
Are there any elegant representations for furious?\\
    \midrule
        
    Base Model ( relevance:2.00 overall:3.87) & 我尝闻宝刀百炼成,可斩离情续旧情。
    
啊,那该是怎样的悲伤才能写成这样的诗句呢?

那就让我变成街道上的一具行尸走肉吧。

    I've heard that \textit{It takes hundreds of times to forge a good knife, and that knife can break up or restore precious past feelings.} 
    
    Oh, how sad it is to write up such a poem?
    
    Please let me be walking dead on the street. \\
    \cdashline{1-2}
    Inverse Prompt ( relevance:4.16 overall:7.65) &  不怒自威,
外强中干,
咆哮不如归去,
怒发冲冠,
怒不可遏,
怒气冲天,
气吞山河,
不可一世,
气急败坏,
咄咄逼人,
怒火中烧。
这些都是能形容愤怒的。只有想不到,没有做不到。
谢邀。欢迎点赞。

Indignation, strong outside weak inside, roar and left, hair stands erect, unstoppable furious, furious to the sky, furious to conquer mountains and rivers, extremely arrogant, utterly discomfited, aggressive, angry. These are all representations for furious. There are only things that you cannot imagine, yet nothing you cannot achieve. Thanks for the invitation and welcome to upvote me.\\
    
    \bottomrule
    \end{tabular}
\end{table}
}

